Fast Algorithms for Packing Proportional Fairness and its Dual

The proportional fair resource allocation problem is a major problem studied in flow control of networks, operations research, and economic theory, where it has found numerous applications. This problem, defined as the constrained maximization of $\sum_i \log x_i$, is known as the packing proportional fairness problem when the feasible set is defined by positive linear constraints and $x \in \mathbb{R}^{n}_{\geq 0}$. In this work, we present a distributed accelerated first-order method for this problem which improves upon previous approaches. We also design an algorithm for the optimization of its dual problem. Both algorithms are width-independent. Finally, we show the latter problem has applications to the volume reduction of bounding simplices in an old linear programming algorithm of (YL82), and we obtain some improvements as a result.

==> definitions_links_global.tex <==
%! TEX root = main.tex
\usepackage{xparse}
\usepackage{xargs} 

\makeatletter % for the arxiv, otherwise the raise link doesn't always work well
\def\Hy@raisedlink@left#1{%
    \ifvmode
        #1%
    \else
        \Hy@SaveSpaceFactor
        \llap{\smash{% \llap{ added
        \begingroup
            \let\HyperRaiseLinkLength\@tempdima
            \setlength\HyperRaiseLinkLength\HyperRaiseLinkDefault
            \HyperRaiseLinkHook
        \expandafter\endgroup
        \expandafter\raise\the\HyperRaiseLinkLength\hbox{%
            \Hy@RestoreSpaceFactor
            #1%
            \Hy@SaveSpaceFactor
        }%
        }}% } to close \llap
        \Hy@RestoreSpaceFactor
        \penalty\@M\hskip\z@ 
    \fi
}
\makeatother


%\newcommand\newlink[2]{{\protect\hyperlink{#1}{\color{black}#2}}}
\newcommand\newlink[2]{{\protect\hyperlink{#1}{\normalcolor #2}}}
\makeatletter
\newcommand\newtarget[2]{\Hy@raisedlink@left{\hypertarget{#1}{}}#2}
\makeatother

\newcommand\linktoproof[1]{{\normalfont[{\hyperlink{proof:#1}{$\downarrow$}}]}}
\newcommand\linkofproof[1]{\newtarget{proof:#1}}

%====

%==== Commands with no links==============================
\DeclareMathOperator{\vol}{vol}
\newcommand{\bigotilde}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}( #1 )}

\newcommand{\defi}{\stackrel{\mathrm{\scriptscriptstyle def}}{=}}

\newcommand{\bigo}[1]{O( #1 )}
\newcommand{\bigol}[1]{O\left( #1 \right)}
\renewcommand{\P}{\mathcal{P}}
\newcommand\oracle{\mathfrak{O}}
\newcommand\x[1]{x^{( #1 )} }
\newcommand\y[1]{y^{( #1 )} }
\newcommand\z[1]{z^{( #1 )} }
\newcommand{\X}{\mathcal{X}}
\newcommand\conv{\operatorname{conv}}
\newcommand\vspan{\operatorname{span}}
\newcommand{\norm}[1]{\| #1 \|} 
\newcommand{\normadj}[1]{\left\| #1 \right\|} 
\newcommand{\abs}[1]{| #1 |} 
\newcommand{\absadj}[1]{\left| #1 \right|} 
\newcommand{\grad}{\nabla} 


\newcommand{\innp}[1]{\langle #1 \rangle}
\newcommand{\ones}{\mathds{1}} 

\usepackage[bb=boondox]{mathalpha} 
\newcommand{\zeros}{\mathbb{0}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\renewcommand{\E}[1]{\mathbb{E}\left[ #1 \right]}
\renewcommand{\R}{\mathbb{R}}
\renewcommand{\D}{\mathcal{D}}
\renewcommand{\P}{\mathcal{P}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\Rp}{\mathbb{R}_{\geq 0}}
\newcommand{\Z}{\mathbb{Z}}
%\newcommand{\N}{\mathbb{N}}

%==== End of commands with links =========================



\let\oldrho\rho
\renewcommand\rho{\newlink{def:rho}{\oldrho}}


\newcommand\N{\newlink{def:N}{N}}
\newcommand\m{\newlink{def:m}{m}}
\newcommand\n{\newlink{def:n}{n}}

\newcommandx*\ecanonical[1][1=i, usedefault]{\newlink{def:e_i_canonical_basis}{e_{#1}}}
\newcommandx*\breg[1][1=\psi, usedefault]{\newlink{def:bregman_div}{D_{#1}}}

\let\oldepsilon\epsilon
\renewcommand\epsilon{\newlink{def:epsilon}{\oldepsilon}}

\let\oldodot\odot
\renewcommand\odot{\newlink{def:entrywise_prod}{\oldodot}}


\newcommand\g{\newlink{def:g}{g}}
\newcommand\f{\newlink{def:f}{f}}

\newcommand\simplex[1]{\newlink{def:simplex}{\Delta^{#1}}}

\newcommand\sign{\newlink{def:sign}{\operatorname{sign}}}

\newcommandx*\xast[1][1= , usedefault]{\newlink{def:xast}{x^\ast_{#1}}}


\newcommand{\YL}{\newlink{def:acronym_yamnitsky_levin}{YL}}
\newcommand{\LP}{\newlink{def:acronym_linear_programming}{LP}}
\newcommand{\PST}{\newlink{def:acronym_plotkin_shmoys_tardos}{PST}}
\newcommand{\MW}{\newlink{def:acronym_multiplicative_weights}{MW}}



